Lattice Simulations of 10d Yang-Mills toroidally compactified to 1d, 2d and 4d

Toroidally compactified Yang-Mills theory on the lattice is studied by using the Hybrid Monte Carlo algorithm. When the compact dimensions are small, the theory naturally reduces to Yang-Mills with scalars. We confirm previous analytical and numerical results for pure gauge theory with scalars in (0+1) dimensions and at high temperatures to Super-Yang-Mills in (1+1) dimensions. In (1+1) dimensions, our simulations confirm the previously conjectured phase diagram. Furthermore, we find evidence for the sequential breaking of the center symmetry in (1+1) dimensions as a function of the volume. In (3+1) dimensions we present first simulation results for the eigenvalue distribution of the Polyakov and Wilson loops, finding localized, non-uniform and center-symmetric configurations as a function of the lattice coupling.

==> numsetup-short.tex <==
%%%%%%%%%%%%%
%%%%%%%%%%%%%
\subsection{Numerical setup}\label{sec:numerical_setup}
%%%%%%%%%%%%%
%%%%%%%%%%%%%

We will be employing a Hybrid Monte Carlo simulation of the {\it quantum} SU(N) Yang-Mills system with arbitrary $N$ for a system in $d$ dimensional Euclidean space-time using standard lattice methods \cite{Montvay:270707}. Our numerical code is publicly available as a service to the community \cite{codedown}.

%%%%%%%%%%%%%
%%%%%%%%%%%%%
%\subsection{Observables}
%\label{sec:lattice}
%%%%%%%%%%%%%
%%%%%%%%%%%%%
As observables we will consider Wilson/Polyakov loops which are defined as $W_i={\cal P}e^{i \oint dx A_i(x)}$ for a loop in the ${\rm i}^{\rm th}$ (Euclidean) direction, where ${\cal P}$ denotes path ordering. On the lattice, this is easily implemented through a product of link matrices
\begin{equation}
W_i=\prod_{m=1}^{m=n_i} U_i(m)\,,
\end{equation}
where $n_i$ denotes the number of lattice sites in the direction i. We will distinguish the case where $i=t$ (the Euclidean ``time'' direction) and $i=(x,y,z)=s$ (one of the Euclidean ``space'' directions), corresponding to the case of Polyakov and Wilson loops, respectively. Of particular interest will be the expectation value of the absolute value of the trace (cf. Ref.~\cite{Catterall:2010fx}),
\begin{equation}
  \label{eq:polyakov}
  \langle P_i \rangle = \left\langle \left|\frac{1}{N}{\rm Tr}\, W_i\right|\right\rangle\,,
\end{equation}
averaged over directions transverse to $i$ and over all configurations. Also, we will study the distribution of eigenvalues $\{e^{i \theta_1},e^{i \theta_2},\ldots,e^{i \theta_N}\}$ of the Wilson/Polyakov loops on the unit circle. The phases of the eigenvalues are required to sum to $2\pi$ times the integer winding number for the SU($N$) gauge group. We will ignore non-trivial topologies in this study and re-center the phases of the eigenvalues so they sum to zero if a non-trivial winding number occurs.
%\footnote{
%\textcolor{red}{
%The detail of the ${\mathbb Z}_N$-fixing procedure is as follows. Let us consider the case of the $t$-direction. 
%Firstly we calculate $\sum_{x,y,z}P_t(x,y,z)$, where $P_t(x,y,z)$ is the Polyakov loop at each spatial point $(x,y,z)$. 
%Then we choose $n_t\in\mathbb{Z}$ so that $e^{2\pi in_t/N}\sum_{x,y,z}P_t(x,y,z)$ becomes as close to real-positive as possible. 
%We determine $n_x, n_y$ and $n_z$ in the same manner. 
%Then, $W_i$'s are re-defined as $W_i\to e^{2\pi in_i/N} W_i$. It fixes the ambiguity of ${\mathbb Z}_N$ configuration by configuration. 
%}}
The distribution of eigenvalue phases on the interval $[-\pi,\pi]$ will then be of interest as an order parameter for the systems considered here.

%Furthermore, we will be interested whether the eigenvalue distribution of the Wilson/Polyakov loop is (approximately) center symmetric or not. If the distribution of $P_i$ is center symmetric, then ${\rm Tr}P_i\simeq 0$, whereas for a completely broken center symmetry we expect ${\rm Tr}P_i\simeq 1$. For finite $N$, the breaking of center symmetry will occur for $0<{\rm Tr}<1$. We define the operator $Z_i$ as an indicator for the presence of the center symmetry of $P_i$ as 
%\begin{equation}
%\label{eq:zidef}
%Z_i\equiv \{\begin{array}{c} 1\quad {\rm if}\quad {\rm Tr}P_i<0.5\\
%0\quad {\rm if}\quad {\rm Tr}P_i>0.5\end{array}
%\end{equation}


Another observable will be the equation of state, e.g. the functional dependence of the energy density $\varepsilon$ on the temperature T. Given a partition function $Z=\int dU e^{-S}$, the energy density and pressure $P$ are calculated as derivatives w.r.t. temperature and volume $V$,
\begin{eqnarray}
  \label{eq:therm1}
  \varepsilon&=&-\frac{1}{V}\frac{\partial \ln Z}{\partial (1/T)}=\frac{T}{V}\left\langle a_t \frac{\partial S}{\partial a_t} \right\rangle \nonumber\\
  P&=&T\frac{\partial \ln Z}{\partial V}=\frac{-T}{(d-1)V}\left\langle a_s \frac{\partial S}{\partial a_s}\right\rangle\,.
\end{eqnarray}
Note that derivatives w.r.t temperature $T=\frac{1}{N_t a_t}$ and volume $V=(N_s a_s)^{d-1}$ for a lattice with a fixed number of sites $N_t,N_s$ in the temporal and spatial directions have been recast as derivatives w.r.t. $a_t,a_s$, the (in principle different) lattice spacings in these directions. For an anisotropic lattice with different lattice spacings in the temporal and spatial directions the action is given by
\begin{equation}
  S=\frac{N^2 a_s^{d-3}}{\lambda_{(d)} a_t}\sum_{x} R_{\rm temp}
  +\frac{N^2 a_t a_s^{d-5}}{\lambda_{(d)}}\sum_{x} R_{\rm spat}\,,
  \end{equation}
where the ``temporal'' and ``spatial'' plaquettes are given as (cf. \cite{Montvay:270707}).
\begin{equation}
  R_{\rm temp}\equiv \sum_{i=1}^{d-1}\left(1-\frac{1}{N}{\rm Re\ Tr\ } U_{ti}\right)\,,\quad
  R_{\rm spat}\equiv \sum_{i=1}^{d-1}\sum_{j>i}^{d-1}\left(1-\frac{1}{N}{\rm Re\ Tr\ } U_{ij}\right)\,.
\end{equation}
Toroidal compactification simply amounts to the replacement $\frac{a_s^{d}}{\lambda_{(d)}}\rightarrow \frac{a_s^{p}}{\lambda_{(p)}}$. 
Away from $p=4$, the coupling is dimensionful and can be scaled away in all physically relevant observables. Thus only the explicit dependence on the lattice spacings contributes to the derivatives in (\ref{eq:therm1}). Setting $a_t=a_s=a$ in the end (isotropic lattice) leads to 
\begin{eqnarray}
  \varepsilon&=&\frac{T}{V} \frac{N^2 a^{p-4}}{\lambda_{(p)}}\sum_x\left(-\langle R_{\rm temp}\rangle +\langle R_{\rm spat}\rangle\right)\,,\\
  P&=&\frac{T}{(p-1)V} \frac{N^2 a^{p-4}}{\lambda_{(p)}}\sum_x\left(-\langle R_{\rm temp}\rangle (p-3)-\langle R_{\rm spat}\rangle (p-5)\right)\,.\nonumber
\end{eqnarray}
As a special case, let us mention that for $p=1$ (matrix model quantum mechanics), we have
\begin{equation}
  \label{eq:E1d}
  \epsilon V = E =\frac{N^2 a^3 T}{\lambda_{(1)}} \sum_x\left(-\langle R_{\rm temp}\rangle +\langle R_{\rm spat}\rangle \right)\,.
  \end{equation}
For $p=4$, in particular, it is advantageous to consider a different strategy to calculate thermodynamic properties. Namely, note that a different definition of the pressure is $P=\frac{T}{V}\ln Z$. Considering
\begin{equation}
  \frac{\partial \ln Z}{\partial \beta_{\rm eff,p}}=-\left\langle \frac{\partial S}{\partial \beta_{\rm eff,p}}\right\rangle
  =-\sum_{x}\left(\langle R_{\rm temp}\rangle +\left\langle R_{\rm spat}\right\rangle \right)\,.
\end{equation}
Integration of this result leads to the pressure. However, care must be taken to remove the zero-temperature contribution. In practice, this is done by subtracting $\langle R_{\rm temp}\rangle +\langle R_{\rm spat}\rangle$ calculated on a lattice with $N_s^D$ sites at each value of $\beta_{\rm eff}$ \cite{Montvay:270707}, 
\begin{eqnarray}
  \frac{P}{T^{D-p}}&=&\int_{\beta_0}^\beta d\bar \beta \Delta S(\bar\beta)\,,\nonumber\\
  \Delta S(\bar \beta)&=&N_t^{D-p}\left[S(N_s,N_s,\bar \beta)-S(N_t,N_s,\bar \beta)\right]\,,\label{eq:deltaS}\\
  S(N_t,N_s,\bar\beta)&\equiv& \frac{1}{N_s^{D-1}N_t} \sum_x \left.\left(\langle R_{\rm temp}\rangle +\langle R_{\rm spat}\rangle\right)\right|_{\bar \beta}\,.\nonumber
  \end{eqnarray}


